Better Algorithms for Individually Fair $k$-Clustering

We study data clustering problems with $\ell_p$-norm objectives (e.g. $k$-Median and $k$-Means) in the context of individual fairness. The dataset consists of $n$ points, and we want to find $k$ centers such that (a) the objective is minimized, while (b) respecting the individual fairness constraint that every point $v$ has a center within a distance at most $r(v)$, where $r(v)$ is $v$'s distance to its $(n/k)$th nearest point. Jung, Kannan, and Lutz [FORC 2020] introduced this concept and designed a clustering algorithm with provable (approximate) fairness and objective guarantees for the $\ell_\infty$ or $k$-Center objective. Mahabadi and Vakilian [ICML 2020] revisited this problem to give a local-search algorithm for all $\ell_p$-norms. Empirically, their algorithms outperform Jung et. al.'s by a large margin in terms of cost (for $k$-Median and $k$-Means), but they incur a reasonable loss in fairness. In this paper, our main contribution is to use Linear Programming (LP) techniques to obtain better algorithms for this problem, both in theory and in practice. We prove that by modifying known LP rounding techniques, one gets a worst-case guarantee on the objective which is much better than in MV20, and empirically, this objective is extremely close to the optimal. Furthermore, our theoretical fairness guarantees are comparable with MV20 in theory, and empirically, we obtain noticeably fairer solutions. Although solving the LP {\em exactly} might be prohibitive, we demonstrate that in practice, a simple sparsification technique drastically improves the run-time of our algorithm.

==> Priority k-Median(3)/abstract.tex <==
\begin{abstract}
We study data clustering problems with $\ell_p$-norm objectives (e.g. \textsc{$k$-Median} and \textsc{$k$-Means}) in the context of individual fairness. The dataset consists of $n$ points, and we want to find $k$ centers such that (a) the objective is minimized, while (b) respecting the individual fairness constraint that every point $v$ has a center within a distance at most $r(v)$, where $r(v)$ is $v$'s distance to its $(n/k)$th nearest point. Jung, Kannan, and Lutz [FORC 2020] introduced this concept and designed a clustering algorithm with provable (approximate) fairness and objective guarantees for the $\ell_\infty$ or \textsc{$k$-Center} objective.  Mahabadi and Vakilian [ICML 2020] revisited this problem to give a local-search algorithm for all $\ell_p$-norms. Empirically, their algorithms outperform Jung et. al.'s by a large margin in terms of cost (for \textsc{$k$-Median} and \textsc{$k$-Means}), but they incur a reasonable loss in fairness. 
In this paper, our main contribution is to use Linear Programming (LP) techniques to obtain better algorithms for this problem, both in theory and in practice. We prove that by modifying known LP rounding techniques, one gets a worst-case guarantee on the objective which is much better than in MV20, and empirically, this objective is extremely close to the optimal.  Furthermore, our theoretical fairness guarantees are comparable with MV20 in theory, and empirically, we obtain noticeably fairer solutions.
Although solving the LP {\em exactly} might be prohibitive, we demonstrate that in practice, a simple sparsification technique drastically improves the run-time of our algorithm.
\end{abstract}

==> Priority k-Median(3)/checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We have provable guarantees}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{In references for the ones named in paper, in comments of the codes for the rest.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Snippets of code. credited in code comments}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> Priority k-Median(3)/conclusion.tex <==
\section{Conclusion}


==> Priority k-Median(3)/experiments.tex <==
\section{Experiments}\label{sec:experiments}

\paragraph{Summary.}
We run experiments to show that the empirical performance of our algorithms can be much superior to the worst-case guarantees claimed by our theorems (the codes are publicly availably on Github\footnote{\url{https://github.com/moonin12/individually-fair-k-clustering}}). While implementing our algorithm, we make the following optimization :
instead of choosing the constant ``$2$'' in \Cref{line:ourR} (definition of $R$) in our algorithm, we perform a binary-search to determine a better constant. Specifically, we find the smallest $\beta$ for which \Cref{alg:filter} gives at most $k$ centers with $R(v) := \min\{r(v), (\beta C_v)^{1/p}\}$ for all $v$. This step is motivated by the experiments in~\cite{JKL20}.


We assess the performance with respect to (a) fairness, (b) objective value, and (c) running times. Due to space restrictions, we focus on the \kmeans objective and leave \kmed results to \Cref{sec:kmedresults}. Our fairness violation seldom exceeds 1.3 (compare this to the theoretical bound of $8$), and often is much better than that of~\cite{MV20} and~\cite{JKL20}. The objective value of our solution is in fact extremely close to the LP solution, which is a {\em lower bound} on the optimum cost (compare this to the theoretical bound of $4$). This occurs because typically the LP solution itself has many integer entries. Finally, although the ``vanilla'' running time of the LP is pretty large, our sparsification routine
\Cref{lma:sparsify} tremendously reduces the running time. 


%TODO include Jung et al datasets
\paragraph{Datasets.} Similar to \cite{MV20}, we use  3 datasets from the UCI repository\footnote{\href{https://archive.ics.uci.edu/ml/datasets/}{https://archive.ics.uci.edu/ml/datasets/}}~\cite{Dua:2019} (also used in previous fair clustsering works of~\cite{CKLV17,BCFN19}). We use a set of numeric features (matching previous work) to represent data in Euclidean metric.\\
 \textbf{1- }\bank~\cite{bank-paper} with 4,521 points, on data collected by the marketing campaign of a Portuguese banking institution. We use 3 features ``age'', ``balance'', and ``duration''.\\
\textbf{2- }\census~\cite{census-paper} with 32,561 points, based on the 1994 US census. Here we use the following 5 features: ``age'' , ``final-weight'', ``education-num'', ``capital-gain'', and ``hours-per-week''.\\
\textbf{3- }\diabetes~\cite{strack2014impact} 
with 101,766 points, from diabetes patient records from 130 hospitals across US.
% \textbf{4- }\censusbig~\cite{meek2002learningcurve} with 2,458,285 points, taken from the 1990 US census with ?? features.

\paragraph{Benchmarks.} We compare with the algorithms of \cite{MV20} and \cite{JKL20}. For~\cite{MV20}, we set parameters according to the experimental section of their paper. We remark that in their experimental section they perform $1$ swap in their local search instead of the $4$-swaps for which they prove their theorem.
% Initially, they run \Cref{alg:filter} but changing the 2 in \Cref{ln:chld} to 3 (as opposed to 6 in their theoretical results), followed by a local search procedure (a modification of~\cite{Arya04,KMN02}) with a single swap. Their theoretical guarantees heavily rely on running this local search with 4 simultaneous swaps, with runtime $\omega(n^4)$ which is infeasible in practice. We also compare with~\cite{JKL20}. 
 For our running time comparison, we also compare ours and the above two algorithm's running times with the 
 popular \kmeanspp algorithm of~\cite{AV07} from scikit learn toolkit~\cite{sklearn} which has no fairness guarantees.
 
 
\subsection{Fairness analysis}\label{subsec:fairness}
For any solution $T\subseteq X$, define the ``violation array'' $\theta_T$ over $v \in X$ as $\theta_T(v) = d(v,T)/r(v)$. This provides a more fine-grained view of the per-client fairness guarantee violation.
Similar to \cite{MV20} we use maximum violation (i.e. $\max_{v \in X}\theta_T(v)$) as a benchmark for fairness. In \Cref{fig:max_violation_main} we have plotted the maximum violation of our algorithm \algoname, \cite{MV20} (noted as MV), and \cite{JKL20} (noted as JKL). We find that our results are noticeably fairer than \cite{MV20} while improving over \cite{JKL20} in many cases.%\footnote{See discussion at the end of \Cref{sec:prelim} and an experimental demonstration in our experimental cost analysis of how this adversely affects their clustering cost.} 

\begin{figure}[!ht]
\includegraphics[height=1.2in]{figures/max_violation/main/bank_1000_maxviolations_aggr.png}
\includegraphics[height=1.2in]{figures/max_violation/main/adult_1000_maxviolations_aggr.png}
\includegraphics[height=1.2in]{figures/max_violation/main/diabetes_1000_maxviolations_aggr.png}
\centering
\caption{Comparison of maximum fairness violation with \kmeans objective, between our algorithm \algoname, the algorithm in \cite{JKL20} (denoted as JKL), and the algorithm in \cite{MV20} (denoted as MV), on average of 10 random samples of size 1000 each.}
\label{fig:max_violation_main}
\end{figure}

Next, we compare the histograms of the violation vectors $\theta$ as described above. This picture provides a better view of the fairness profile, as just looking at the maximum violation may not be a robust measure;  an algorithm that is largely unfair may be preferred to an algorithm that is extremely unfair on a single point but extremely fair on all the rest. We show the histograms of the violation vectors of these algorithms in \Cref{fig:violation_hist_main} (for a full set of histograms see \Cref{subsec:means_histograms}). As an example, even though in \bank with $k=20$ our maximum violation is slightly worse than \cite{JKL20} our histogram shows that we are slightly fairer overall. We observe that our algorithm ensures complete fairness for at least \%80 of the points in almost all the experiments. A theoretical study of the violation vector is interesting and left as future work.
\begin{figure}[!ht]
\includegraphics[height=1.2in]{figures/violation_histogram/main/bank_1000_radii_violations_aggr_20_jkl.png}
\includegraphics[height=1.2in]{figures/violation_histogram/main/bank_1000_radii_violations_aggr_20_mv.png}
\centering
\caption{Histograms of violation vectors on \bank with $k=20$ \kmeans objective comparing \algoname with the algorithm in \cite{JKL20} (denoted as JKL) and the algorithm in \cite{MV20} (denoted as MV), on average of 10 random samples of size 1000 each.}
\label{fig:violation_hist_main}
\end{figure}

\subsection{Cost analysis}\label{subsec:cost}
In \Cref{fig:cost-main} we demonstrate that in our experiments, the objective value almost matches the optimal cost, begin at most \%1 more almost always, and never above \%15 more than the LP cost.
%As mentioned earlier, \cite{JKL20} cost is much higher than any of the other benchmarks. 
Note that our cost is also {\em higher} than that of \cite{MV20}, and the reader may be wondering how the latter can be better than the optimum cost. The reason is that the \cite{MV20} cost is violating the fairness constraint while the optimal cost is not. To do a more apples-to-apples comparison, one can also allow the same violations as~\cite{MV20} and re-solve the linear program and also our rounding algorithms. On doing so, we do find that our algorithm's cost becomes lower than that of~\cite{MV20}.
Details of this can be found in~\Cref{subsec:rel_plots}.
The set-up also allows us to measure the \emph{cost of fairness}: how much does the linear programming cost and our algorithm's cost decrease as we relax the fairness constraints. We do this empirical study; see \Cref{subsec:cost_of_fairness} for our results.


% we argue that this is unavoidable for ensuring our level of fairness for two reasons: One, the optimal solution itself closely matches ours and two, allowing the same violations as \cite{MV20} drops our cost to the same level as \cite{MV20}. To be precise, let $T$ be the \cite{MV20} solution and define $r'$, the \emph{relaxed} fairness radii, as $r'(v) := \max\{d(v,T), r(v)\}$. Then solve the LP on the relaxed radii and we get a lower-bound on the cost of any $r'$-fair solution. Furthermore, we use this LP-solution to run \algoname (call it \relalgoname) and observe that its radii violations and cost almost match~\cite{MV20} (see \Cref{subsec:rel_plots}).

\begin{figure}[!ht]
\includegraphics[height=1.2in]{figures/subsamp_costs/main/bank_1000_costs_aggr.png}
\includegraphics[height=1.2in]{figures/subsamp_costs/main/adult_1000_costs_aggr.png}
\includegraphics[height=1.2in]{figures/subsamp_costs/main/diabetes_1000_costs_aggr.png}
\centering
\caption{Comparison of \kmeans clustering cost, between our algorithm \algoname, the algorithm in \cite{JKL20} (denoted as JKL), and the algorithm in \cite{MV20} (denoted as MV), on average of 10 random samples of size 1000 each.  We also plot the LP cost which is a lower bound on the optimum cost (denoted as {\sf Fair-LP}.}
\label{fig:cost-main}
\end{figure}


%\Cref{fig:cost_of_fairness_main} shows how the fair LP cost approaches the \kmeans cost as fairness radii is relaxed. % Then run experiments to demonstrate ``cost of fairness'' that only includes fair LP, vanilla LP, and vanilla clustering

\paragraph{Runtime analysis.} We run our experiments in Python 3.8.2 on a MacBook Pro with 2.3 GHz 8-Core Intel Corei9 processor and 32 GB of DDR4 memory. 
 We solve our linear programs  using the Python API for CPLEX~\cite{CPLEX}.
We demonstrate that even though solving an LP on the entire instance is time consuming, our sparsification step tremendously improves on the runtime (\Cref{fig:time_main}) while increasing the clustering cost or fairness performance by a only a negligible margin (see \Cref{subsec:spa_plots} for the cost and fairness results). Below, the blue line with circles shows \algoname with ``vanilla'' LP solver, and the green line with upside-down triangles \spaalgoname is the runtimes with the sparse LP solution.

\begin{figure}[!ht]
\includegraphics[height=1.2in]{figures/time/main/bank_1000_times_aggr.png}
\includegraphics[height=1.2in]{figures/time/main/adult_1000_times_aggr.png}
\includegraphics[height=1.2in]{figures/time/main/diabetes_1000_times_aggr.png}
\centering
\caption{Comparison runtime with \kmeans objective, between our algorithm \algoname, the algorithm in \cite{JKL20} (denoted as JKL), the algorithm in \cite{MV20} (denoted as MV), and \kmeanspp on average of 10 random samples of size 1000 each. Here, $\delta = 0.3$, $0.05$ and $0.01$ for \bank, \census, and \diabetes. Note that \cite{JKL20}, \kmeanspp, and our sparsified algorithm \spaalgoname have very small differences in their running times.}
\label{fig:time_main}
\end{figure}




==> Priority k-Median(3)/intro.tex <==
\section{Introduction}
As machine learning algorithms are widely used in practice for making high-stakes decisions affecting human lives, there has been a huge body of work on {\sc Fair-ML} trying to ensure `fairness' in the solutions returned by these algorithms. 
%
% such as awarding home loans~\cite{khandani2010consumer,malhotra2003evaluating} and predicting recidivism in court~\cite{propublica,dressel2018accuracy,chouldechova2017fair}, it is imperative to make sure these algorithms are \emph{fair}. 
There are two large intersecting bodies of work : one body's main focus in to understand what `fairness' means
 (e.g.~\cite{kamishima2012fairness,zemel2013learning,ZafarVGG17,yang2017measuring,CKLV17,JKL20}) in various different contexts, and the second body's focus has been on addressing the {\em algorithmic challenges} brought forth by these considerations (e.g.,~\cite{joseph2016fairness,celis2018,RS18,BCFN19,MV20,BCCN21}). 
 
%  . Among learning algorithms, clustering is a fundamental unsupervised method and there is specifically a line of research on fair clustering algorithms including~\cite{RS18,CKLV17,BCFN19,JKL20,MV20,BCCN21}. 
This paper falls in the second class. In particular, we consider an {\em individual fairness} model proposed by Jung, Kannan, and Lutz~\cite{JKL20} for a $k$-clustering problem. Given points (clients) $X$ in a space with metric distance $d$, find $k$ points (facilities) $S\subseteq X$, minimizing \cost where $d(v,S)$ is $v$'s distance to the closest point in $S$. This includes \kcent, \kmed and the popular \kmeans objective for $p=\infty$, $p=1$ and $p=2$ respectively, problems which have been extensively studied~\cite{CGST99,JV99,kanungo2002efficient,AV07,ANSW17} in the algorithms literature. Jung et. al.~\cite{JKL20} proposed that in this context a solution would be deemed individually fair, if for every client $v\in X$
there is an open facility not too far from it. More precisely, if there is a facility within distance $r(v)$ which is the smallest radius around $v$ that contains $n/k$ points. The rationale behind $n/k$ is that every facility, on average, serves $n/k$ clients.

Jung et al.~\cite{JKL20} gave a solution where every client $v$ was served within a radius of $2r(v)$, which as a jargon is called $2$-approximate fair solution. However, their solution did not explicitly consider the ``objective'' function (\kmeans/\kmed, for instance) in the clustering problem, which is often used as a proxy to measure the quality of the clustering. This was addressed in a follow up paper by 
Mahabadi and Vakilian~\cite{MV20} who gave a $(7,O(p))$-approximation with respect to the \lpnorm objective. That is, they give a local-search based solution which is $7$-approximately fair, but the objective is violated by some $Cp$-factor where the constant $C$ is rather large (for $p=1$, the factor is $84$). The theoretical running time of their algorithm is $\Tilde{O}(pk^5n^4)$.

\subsection{Our Contributions}\label{subsec:contribution}

The main contribution of our paper is to give improved algorithms for this problem using {\em linear programming rounding}. Our study stems from two observations: one, that the problem at the core of Jung et al.~\cite{JKL20} was in fact studied as ``weighted/priority \kcent problem'' by Plesn\'ik\cite{Ples87}, and that if all the $r(v)$'s were the same (which may not at all be the case), then the clustering problem has also been studied under the guise of centridian/ordered median problem~\cite{AS17,BSS18,CS18}. Combining ideas from these two bodies of work, we design an $(8,8)$ algorithm for the \pkmed problem, which obtains an $8$-approximation for both cost and fairness (our cost guarantees improve as $p$ grows). 

\begin{itheorem}
There is an $(8,\ourbeta)$-approximation algorithm for \ppkc that runs in LP solving time plus $\Tilde{O}(n^2)$, overall $\Tilde{O}(kn^4)$. In particular, we have 
$(8,8)$-approximation and $(8,4)$-approximation algorithms for \pkmed and \pkmeans, respectively.
\end{itheorem}

Although solving an LP may seem prohibitive in practice, we can obtain a much faster running time by implementing a {\em sparsification} routine (inspired by \cite{Ples87,hs85}) with a marginal hit in the fairness and clustering cost (see \Cref{lma:sparsify} for details). Empirically, this greatly decreases the running time, and is often faster than the~\cite{MV20} implementation.

In our experiments, we also find that our theoretical bounds are too pessimistic. 
Indeed, we show that our algorithm's cost is at most \%1 more than the {\em optimal} clustering cost (which does not have any fairness violation), almost always, and never more than \%15 in the rest. Furthermore, our maximum fairness violation is at most a factor of 1.27 which is much better than our theoretical guarantee of 8. We also do a more fine-grained analysis of the fairness violation : consider a vector where each coordinate stands for a clients ``unfairness'' indicating the ratio of its distance to $r(v)$. When we plot this as a histogram, we find that most of the mass is shifted to the ``left'', that is, the percentage of clients who satisfy their fairness constraints is significantly larger than in the~\cite{MV20} solution. This seems to suggest the linear program, which is trying to minimize the cost, itself tries to increase the number of fairly treated clients. We leave a theoretical investigation of this phenomenon for future work.

Our experiments also demonstrate the {\em price of fairness}. We find that our linear programs, which maintains absolute fairness, have objective value considerably larger than that of~\cite{MV20}. On the other hand, if we tune the ``fairness violation'' of the linear program to match that of~\cite{MV20}, then the objective value of our algorithm drops. 
% In practice, our output is noticeably fairer than \cite{MV20} but still less fair compared to~\cite{JKL20}. Of course ~\cite{JKL20} cost for both \kmed and \kmeans is considerably worse than our cost and~\cite{MV20}'s. In fact, even our cost seems to be worse than~\cite{MV20} by a margin. We demonstrate, that this is the price we pay for better fairness: If we allow the exact same fairness violations as~\cite{MV20} our clustering cost drops, almost matching \cite{MV20} and the optimal cost for this \emph{relaxed} \ppkc instance. 
We run experiments to further elaborate on the inherent \emph{cost of fairness} in our datasets by demonstrating how the optimal cost changes with respect to varying degrees of fairness relaxation.

It is worth noting that our algorithm works for arbitrary values of $r(v) \geq 0$ for points $v$ (and this may be true for~\cite{MV20} as well), and we present our results thus. This setting might be of interest in applications where the ``fair radius'' may not be $n/k$ but something more nuanced. 


\subsection{Other related work}

\kcent has a 2-approximation due to Gonzales, and Hochbaum and Shmoys~\cite{Gon85,hs85} and they prove it is NP-hard to get better approximations. \kmed, and \kmeans are hard to approximate within factors better than 1.73 and 3.94~\cite{GK98} respectively with current best approximations being 2.67 by~\cite{BPRS14} and 9 by~\cite{ANSW17}. Also recently, there has been an improvement on lower-bounds for approximating \emph{Continuous} \kmed and \kmeans where centers can be picked anywhere in the real space. By Cohen-Addad, Karthik, and Lee~\cite{CCL21}, it is NP-hard to approximate Continuous \kmed and \kmeans within factors $2-o(1)$ and $4-o(1)$ respectively.

\pkcent is a special case of \emph{Priority} \kcent where the radii $r(v)$ in which a point $v$ demands a center at that distance, are general values. \cite{Ples87} introduced this problem and gave a best possible 2-approximation. G{\o}rtz and Wirth~\cite{GW06} study the problem for asymmetric metrics and prove that it is NP-hard to obtain any non-trivial approximation. \cite{BCCN21} give a 9-approximation for the problem in presence of \emph{outliers} and further generalize to constant approximations for general constraints on the solution centers. Another very closely related problem is \emph{Chance-$k$-Coverage} introduced in~\cite{HLPST19} in which for any point $v$, in addition to $r(v)$, a probability $p(v)$ is given and the goal is to find a distribution on possible solutions such that a solution drawn from this distribution covers $v$ with probability at least $p(v)$. This also has a 9-approximation by \cite{HLPST19}.

A clustering problem related to \pkmed and \pkmeans is the \emph{Simultaneous $k$-Clustering} in which the goal is to find a solution with approximation guarantees with respect to any monotone, symmetric norm. This problem has an $O(1)$-approximation due to Chakrabarty and Swamy~\cite{CS19} with a line of previous work including~\cite{AS17,CS18,BSS18}.

Another similar notion of individual fairness is introduced by Chen et al.~\cite{ChenFLM19} in which a solution is fair if there is no group of size at least $n/k$ for which there exists a facility that would reduce the connection cost of all members of the group if opened. \cite{ChenFLM19} give a $(1+\sqrt{2})$-approximation for $\ell_1$, $\ell_2$, and $\ell_\infty$ norm distances for the setting where facilities can be places anywhere in the real space. Micha and Shah~\cite{MS20} modified the approach to give close to 2-approximation for $\ell_2$ and proved the previous results for $\ell_1$ and $\ell_\infty$ are indeed tight.



==> Priority k-Median(3)/mainalgo.tex <==
\section{Algorithm for \ppkc problem}

Now we are ready to describe our algorithm \algoname which establishes~\Cref{thm:main}. 
At a high-level, we run our \filter routine  by defining the input function $R$ in a manner that is conscious of the \ppkc cost: given $(x^*,y^*)$ which is an optimal solution to \eqref{lp:ppkc}, for any $v \in X$ let $C_v$ be $v$'s contribution to the \ref{lp:ppkc} cost i.e. $C_v := \sum_{u \in X}d(v,u)^px^*_{vu}$ and define $R(v) := \min\{r(v), (2C_v)^{1/p}\}$. Let us ponder for a bit to see what changes from \Cref{thm:ples}. For the output $S$, we still have the fairness guarantee $d(v,S) \leq 2r(v)$ for all $v$ but since $(2C_v)^{1/p}$ might be less than $r(v)$ for any $v$, we cannot guarantee that $|S| \leq k$. Thankfully, in this case, we can still prove $|S| \leq 2k$ (\Cref{cor:s2k}). The rest of the algorithm is deciding on a subset of at most $k$ points out of this $S$ to return as the final solution, while ensuring the fairness and cost guarantees are still within constant factor of the optimal. This idea is very similar to existing ideas in~\cite{AS17,CGST99} which look at the problem without fairness considerations.

Recall that $\{D(u) : u \in S\}$ partitions $X$ and each $u \in S$ is responsible for covering all the points in $D(u)$. Here, we could simply move each point in $D(u)$ to $u$ and divert the $y$ value of each point to its closest point in $S$. Note that, $y(S) = k$ (\Cref{fact:yisk}) and similar to the proof of \Cref{thm:ples} we could show $y_u \geq 1/2$ (\Cref{lma:halftoone}) for all $u \in S$ hence $|S| \leq 2k$ (\Cref{cor:s2k}). If this leads to some $y$-value reaching $1$, we open those centers.

For $u \in S$ with $y_u < 1$, if we do not decide to include it in the final solution, we promise to open $S_u$, its closest point in $S$ other than itself. In this case, all the $|D(u)|$ points on $u$ are delegated to $S_u$. Using the fact that $y_u < 1$, we can prove that fairness guarantee (\Cref{lma:kcentapx}) approximately holds for the points in $D(u)$ even after this delegation.

To get the clustering cost guarantee, we need to do more work. Observe that, currently, $u$ is already fractionally assigned to $v$ by $1-y_u$. So if instead of $y_u \geq 1/2$ we had $y_u = 1/2$ we could ensure that already $u$ is assigned to $v$ by $1/2$ thus integrally assigning $u$ to $v$ only doubles the cost. This is why we need to do more work to get $y_u \in \{1/2,1\}$ for $u \in S$ (see \Cref{lma:halfint}) and then bound the clustering cost in \Cref{lma:kmedapx}. 

\begin{algorithm}[!ht]
	\caption{\algoname: \ppkc bi-criteria approximation}
	\label{alg:main}
	\begin{algorithmic}[1]
		\Require Metric $(X,d)$, radius function $r: X \to \Rset^+$, and $(x^*,y^*)$ an optimal solution of \ref{lp:ppkc}
		\State $C_v \leftarrow \sum_{u \in X}d(v,u)^px^*_{vu}\quad \forall v \in X$\Comment{$v$'s cost share in the \ref{lp:ppkc} objective}
		\State $R(v) \leftarrow \min\{r(v), (2C_v)^{1/p}\}\quad \forall v \in X$\label{line:ourR}
		\State $S, \{D(u) : u \in S\} \leftarrow \filter((X,d),R)$
		\If{$|S| \leq k$}
		    \State \Return $S$
		\EndIf
		\State $(x,y) \leftarrow (x^*,y^*)$
% 		\For{all $u \in S$}\Comment{For all $u \in S$, direct $y$ mass from $B(u,R(u))$ to $u$}
% 		    \State $y_u \leftarrow y_u + y(B(u,R(u)))$ \Comment{Note: May cause $y_u$ to increase above 1}
% 		    \State $y_v \leftarrow 0 \quad \forall v \in B(u,R(u))$
% 		\EndFor\label{ln:move-core}
		\For{all $v \in X\backslash S$}\Comment{Direct $y$ mass from outside of $S$ to the closest point in $S$}
		    \State $u \leftarrow $ closest point in $S$ to $v$
		    \State $y_u \leftarrow y_u + y_v$, $y_v \leftarrow 0$ \Comment{Note: May cause $y_u$ to increase above 1}
		\EndFor\label{ln:move-rest}
		\While{There are $u,v \in S$ with $y_u > 1$ and $y_v < 1$}\Comment{Ensure $y_u \leq 1$ for all $u \in S$}
	        \State $y_u \leftarrow y_u - \delta$, $y_v \leftarrow y_v + \delta$, where $\delta := \min\{1-y_v, y_u-1\}$
	    \EndWhile\label{ln:smudge} \Comment{Remark: By now, $ 1/2 \leq y_u \leq 1$ for all $u \in S$ (see \Cref{lma:halftoone}).}
	    \State $S_u \leftarrow $ closest point in $S\backslash u$ to $u$  $\quad \forall u \in S$
	    \While{There are $u,v \in S$ with \\\qquad$1/2 < y_u < 1$, and $y_v < 1$,\\\qquad$d(u,S_u)^p|D(u)| > d(v,S_v)^p|D(v)|$} \Comment{Move $y$ mass from $u$ to $v$ if $u$ is costlier }
	        \State $y_u \leftarrow y_u - \delta$, $y_v \leftarrow y_v + \delta$, where $\delta := \min\{1-y_v, y_u-1/2\}$
	    \EndWhile\label{ln:halfint}\Comment{Remark: At this point, $y_u \in \{1/2,1\}$ for all $u \in S$ (see \Cref{lma:halfint}).}
	    \State $T \leftarrow u \in S$ with $y_u = 1$
	    \State Consider the forest of arbitrary rooted trees on vertices $u \in S$ with edges $(u,S_u)$. Let $O$ be odd-level vertices in $S\backslash T$, and $E$ be even-level vertices in $S\backslash T$.
	    \If{$|E| \leq |O|$} 
	        \State $T \leftarrow T \cup E$
	    \Else
	        \State $T \leftarrow T \cup O$
	   \EndIf
		\Ensure $T$
	\end{algorithmic}
\end{algorithm}

\begin{fact}\label{fact:yisk}
$y(S) = k$ and remains so after \Cref{ln:move-rest}.
\end{fact}
%deepc: I think this can be removed
% \begin{proof}
% We initialize $y$ to $y^*$ for which $y^*(X) = k$ by \ref{lp:budget}. The algorithm then transfers $y(X)$ to $S$ by \Cref{ln:move-rest} without changing the total. Afterwards, the total value of $y(S)$ is unchanged.
% \end{proof}
\begin{lemma}\label{lma:halftoone}
After \Cref{ln:smudge} of \Cref{alg:main}, $ 1/2 \leq y_u \leq 1$ for all $u \in S$.
\end{lemma}
\begin{proof}
First we argue that $y_u \geq 1/2$ for all $u \in S$ by the end of \Cref{ln:move-rest}. Fix $u \in S$. Per \Cref{fact:coreinside} $y(B(u,R(u)))$ is entirely moved to $y_u$. By definition of $R(u)$ there are two cases: Case I, $R(u) = r(u)$ thus $y_u \geq 1$ as $y^*(B(v,r(v))) \geq 1$ for all $v \in X$ according to \Cref{fact:lpyis1}. Case II, $R(u) = (2C_u)^{1/p}$ then by Markov's inequality $y^*(B(u,R(u))) \geq 1/2$ and after this point, $y_u$ is never decreased to below $1/2$. 
More precisely, 
%Let us elaborate on the Markov inequality.
%\begin{equation*}
 $  C_u = \sum_{v \in X}d(u,v)^px^*_{uv} \geq \sum_{\substack{v \in X:\\ d(u,v)>R(u)}}d(u,v)^px^*_{uv} \geq 2C_u\sum_{\substack{v \in X:\\ d(u,v)>R(u)}}x^*_{uv}$.
%\end{equation*}
Considering $\sum_{v \in X}x^*_{uv} = 1$ by \ref{lp:cover}, this implies $\sum_{\substack{v \in X:\\ d(u,v)\leq R(u)}}x^*_{uv} \geq 1/2$ thus $y^*(B(u,R(u))) \geq 1/2$.

As for proving $y_u \leq 1$, it might indeed be the case that $y_u > 1$ by the end of \Cref{ln:move-rest} but the loop ending at \Cref{ln:smudge} can guarantee $y_u \leq 1$ for all $u \in S$. This is because $y(S) = k$ (\Cref{fact:yisk}) and we already checked in the beginning of \Cref{alg:main} that $|S| > k$.
\end{proof}
\begin{corollary}\label{cor:s2k}
 $S$ in \Cref{alg:main} has size at most $2k$.
\end{corollary}
% \begin{proof}
% $y(S) = k$ by \Cref{fact:yisk} and $y_u \geq 1/2$ for all $u \in S$ thus $|S| \leq 2k$.
% \end{proof}

\begin{lemma}\label{lma:halfint}
After \Cref{ln:halfint} of \Cref{alg:main}, $y_u \in \{1/2,1\}$ for all $u \in S$.
\end{lemma}
\begin{proof}
Suppose not. Since $y(S) = k$ (\Cref{fact:yisk}) and $k$ is an integer, by \Cref{lma:halftoone}, there has to be at least two $u,v \in S$ with $y_u,y_v \in (1/2,1)$ which is a contradiction, since either one of them has to be changed to $1/2$ or 1 in the while loop ending at \Cref{ln:halfint}.
\end{proof}

\begin{lemma}\label{lma:kcentapx}
For all $v \in X$, $d(v,T) \leq 8r(v)$.
\end{lemma}
\begin{proof}
Fix $v \in X$. Since $\{D(u) : u \in S\}$ partitions $X$ there exists $u \in S$ such that $v \in D(u)$. According to \Cref{fact:filter} $d(v,u) \leq 2R(v) \leq 2r(v)$ by definition of $R$. If $u$ ends up in $T$ we are done. Else, it has to be that $y_u < 1$ and $S_u \in T$. In what follows, we prove that if $y_u < 1$ at \Cref{ln:halfint} then $d(u,S_u) \leq 6r(v)$. This implies $d(v,S_u) \leq 8r(v)$ hence the lemma.

We know that initially $y^*(B(v,r(v))) \geq 1$ per \Cref{fact:lpyis1} but since $v \notin S$, the $y$ mass on $B(v,r(v))$ has been moved to $S$ by \Cref{ln:move-rest}. If for all $w \in B(v,r(v))$ their closest point in $S$ was $u$, all of $y(B(v,r(v)))$ would be moved to $u$ then $y_u = 1$ by the end of \Cref{ln:halfint}. So there must exist $w \in B(v,r(v))$ with $x^*_{vw} > 0$ along with $u' \in S$, $u' \neq u$, such that $d(w,u') \leq d(w,u)$ which made $y_w$ to be moved to $u'$. By definition of $S_u$, $d(u,S_u) \leq d(u,u')$. Applying the triangle inequality twice gives:
\begin{alignat}{6}
    d(u,S_u) &&~\leq~& d(u,u') \leq d(u,w) + d(w,u') &&~\leq~&& 2d(u,w) \notag \\
    &&~\leq~& 2(d(u,v) + d(v,w)) &&~\leq~&& 2(2r(v) + r(v)) = 6r(v)\notag
\end{alignat}
where the last inequality comes from \Cref{fact:filter} stating $d(u,v) \leq 2r(v)$, and from the fact that $x^*_{vw} > 0$ implies $d(v,w) \leq r(v)$ by \ref{lp:connect}.
%this para is probably not helpful
% Note that, one can also prove $d(u,S_u) \leq 2r(u)$ by similar analysis, looking at a $w$ for which $x^*_{uw} >0$ and $y_w$ was moved to $u' \in S$ other than $u$. That is $d(u,S_u) \leq d(u,u') \leq d(u,w) + d(w,u') \leq 2d(u,w) \leq 2r(u)$. If it was true that $r(v) \leq r(u)$ (in particular for uniform $r$) this would imply $d(v,T) \leq 4r(v)$. This is precisely how~\cite{AS17} get their fairness guarantee of 4 for uniform $r$.
\end{proof}
\begin{lemma}\label{lma:kmedapx}
$\big(\sum_{v \in X} d(v,T)^p\big)^{1/p} \leq \big((2^{p+2})\sum_{v,u \in X}C_v\big)^{1/p} \leq \ourbeta\opt$.
\end{lemma}
\begin{proof}
For the proof, we compare $\sum_{v \in X} d(v,T)^p$ with the optimal \ref{lp:ppkc} cost $\sum_{v \in X} C_v$ which is at most $\opt^p$. Fix $v \in X$ and $u \in S$ for which $v \in D(u)$. By \Cref{fact:filter} $d(v,u) \leq 2R(v) \leq 2(2C_v)^{1/p}$ per definition of $R$. So moving $D(u)$ to $u$ for all $u \in S$ has an additive cost of $\sum_{u \in S}\sum_{v \in D(u)} d(v,u)^p \leq 2^{p+1} \sum_{v \in X} C_v$. From now on, assume there are $D(u)$ collocated points on a $u \in S$.

Moving around the $y$ mass up to \Cref{ln:move-rest} adds a multiplicative factor of $2^p$ loss in the approximation ratio. The logic is: if $u \in S$ was relying on $w \in X$ in the \ref{lp:ppkc} solution, meaning, $x^*_{uw} > 0$ and $y_w$ was moved to a $u' \in S$ (due to $d(w,u') \leq d(w,u)$) then the cost $u$ has to pay to connect to $u'$ is $d(u,u')^p \leq (d(u,w) + d(w,u'))^p \leq 2^pd(u,w)^p$ which is a $2^p$ factor worse than the \ref{lp:ppkc} cost $d(u,w)^p$ it was paying to connect to $w$ earlier.

At this point (\Cref{ln:smudge}), note that the cost incurred by $u$ is $|D(u)|d(u,S_u)^p(1-y_u)$. To elaborate on this, corresponding to $y$, we define an $x$ such that $(x,y)$ is feasible for \ref{lp:ppkc}. Let $x_{uu} = y_u$ and $x_{uS_u}= 1-y_u$ so that \ref{lp:connect} is satisfied for $u$. Then the cost incurred by u is $|D(u)|(d(u,u)^px_{uu} + d(u,S_u)^px_{uS_u}) = |D(u)|d(u,S_u)^p(1-y_u)$. The while loop ending at \Cref{ln:halfint} does not increase the value of the objective function: As we decrease $y_u$ and increase $y_v$, only if the cost incurred by $u$ is bigger than that of $v$. The last multiplicative factor 2 loss comes from when $u \in S\backslash T$. In which case, $y_u = 1/2$ and $S_u \in T$. So by assigning $u$ to $S_u$ we pay $|D(u)|d(u,S_u)^p$ which is twice more than before (as $1-y_u  =1/2$). Observe that this last step is why we needed to do all the work to get $y_u \in \{1/2,1\}$ in \Cref{lma:halfint}. Putting the three steps together, the overall cost is at most $2\times2^p+2^{p+1} = 2^{p+2}$ times the \ref{lp:ppkc} cost or at most $\ourbeta\opt$.
\end{proof}


\begin{proof}[Proof of \Cref{thm:main}]
Using \Cref{cor:s2k} and the fact that $|T| \leq |S|/2$ by construction, we have $|T| \leq k$. \Cref{lma:kcentapx,lma:kmedapx} give the fairness and approximation guarantees. As for runtime, notice that \Cref{alg:main} runs in time $\Tilde{O}(n^2)$. But the runtime is dominated by the \ref{lp:ppkc} solving time. According to \cite{Young01}, finding a $(1+\varepsilon)$-approximation to \ref{lp:ppkc} takes time $O(kn^2/\epsilon^2)$. Setting $\varepsilon = 1/n$ gives the $O(kn^4)$ runtime.
\end{proof}


As evident, the runtime is dominated by the \ref{lp:ppkc} solving time. We end this section by descibing the sparsification pre-processing that when applied to the original instance, can tremendously decrease the \ref{lp:ppkc} solving time in practice while incurring only a small loss in fairness and clustering cost. One reason why the LP takes a lot of time is because there are many variables; $x_{vu}$ for every $v\in X$ and every $u$ within distance $r(v)$ of $v$. To fix this, we first run the \filter algorithm on the data set with $R(v) = \delta r(v)$, where $\delta$ is a tune-able parameter. It is not too hard to quantify the loss in fairness and cost as a function of $\delta$, and we do so in the lemma below. More importantly, note that when $\delta = 1$, then the number of variables goes down from $n$ to $O(k)$; this is because of the definition of $r(v)$ which guarantees $\approx n/k$ points in the radius $r(v)$ around $v$. Therefore, running the pre-processing step would make the number of remaining points $\approx k$. In our experiments we set $\delta$ to be much smaller, and yet observe a great drop in our running times.

\begin{algorithm}[!ht]
	\caption{Sparsification + \algoname}
	\label{alg:sparsemain}
	\begin{algorithmic}[1]
		\Require Metric $(X,d)$, radius function $r: X \to \Rset^+$, parameter $\delta > 0$
		\State $S, \{D(u) : u \in S\} \leftarrow \filter((X,d),\delta r)$
		\State $(x',y') \leftarrow$ solve \ref{lp:ppkc} only on points $S$ with objective function $\sum_{v,u \in S} d(v,u)^px_{vu}|D(v)|$
		\State $ x^*_{vw} \leftarrow x'_{uw}\forall v,w \in X, u\in S: v\in D(u)$\Comment{$v$'s assignment is identical to its representative $u$}
		\State $y^*_u \leftarrow y'_u$ if $u \in S$ and 0 otherwise
		\Ensure $\algoname((X,d),(1+\delta) r,(x^*,y^*))$
	\end{algorithmic}
\end{algorithm}

\begin{lemma}\label{lma:sparsify}
\Cref{alg:sparsemain} outputs an $(8(1 + \delta), \ourbeta(1 + (\delta\phi)^p)^{1/p})$-approximation where $\phi = (\sum_{v \in X}r(v)^p)^{1/p}/\opt$.
\end{lemma}
\begin{proof}
Observe that $(x^*,y^*)$ is not a feasible \ref{lp:ppkc} solution anymore. Nevertheless, it will be feasible for when $r$ is dilated by a factor of $(1+\delta)$ in the \ref{lp:connect}. Here is how we argue \ref{lp:connect} holds in this case: For any $v,w \in X$ for which $x^*_{vw} > 0$,  recall $u \in S$ is chosen so $v \in D(u)$ and $x^*_{vw} := x'_{uw} > 0$ meaning $d(u,w) \leq r(u)$. We have $d(v,w) \leq d(v,u) + d(u,w) \leq \delta r(v) + r(u) \leq (1+\delta)r(v)$. The last two inequalities are by \Cref{fact:filter} as $d(v,u) \leq \delta r(v)$ and $r(u) \leq r(v)$. As for the \ref{lp:ppkc} cost of $(x^*,y^*)$, it is not longer upper-bounded by $\opt^p$ but rather by $\opt^p + \sum_{u \in S}\sum_{v\in D(u)}d(v,u)^p$. This additive term is at most $\sum_{v \in X}(\delta r(v))^p \leq (\delta\phi\opt)^p$. Plugging this into \Cref{lma:kmedapx} finishes the proof.
\end{proof}



==> Priority k-Median(3)/prelim.tex <==
\section{Preliminaries}\label{sec:prelim}
In this section, we formally define our problems, establish some notations, and describe a classic clustering routine due to Hochbaum and Shmoys~\cite{hs85} with modifications by Plesn\'ik\cite{Ples87}. 
Given a subset $S\subseteq X$, we use
$d(v,S)$ to denote  $v$'s distance to the closest point in $S$.

\begin{definition}[\ppkc Problem]
  The input is a metric space $(X,d)$, radius
  function $r: X \to \Rset^+$, and integers $p,k \geq 1$. The goal is to find $S \subseteq X$ of size at most $k$ such that $d(v,S) \leq r(v)$ for all $v \in X$ and the clustering cost \cost is minimized.
\end{definition}

Let $\opt$ be the clustering cost of an optimal solution. For $\alpha,\beta \geq 1$, an $(\alpha,\beta)$-approximate solution is $S \subseteq X$ of size at most $k$ with $d(v,S) \leq \alpha r(v)$ for all $v\in X$ and \cost$ \leq \beta\opt$. In plain English, the fairness approximation is $\alpha$ while the objective/cost approximation is $\beta$.
Our main result is the following.


\begin{theorem}\label{thm:main}
There is an $(8,\ourbeta)$-approximation algorithm for \ppkc that runs in LP solving time plus $\Tilde{O}(n^2)$, overall $\Tilde{O}(kn^4)$.
\end{theorem}

\noindent
The algorithm relies on rounding a solution to the following LP for \ppkc\footnote{The LP and its rounding is slightly different for $p=\infty$; we omit this from this version.} where the optimal \ref{lp:ppkc} objective is at most $\opt^p$. The variable $y_u$ denotes the amount by which $u \in X$ is open as a center. $x_{vu}$ for $v,u \in X$ is the amount by which $v$ is assigned to $u$. The constraints respectively capture the conditions: every client must connect to someone, $k$ centers are opened, no client can connect to an unopened center, and crucially that a client cannot travel to a center further than $r(v)$.

\begin{minipage}{0.55\textwidth}
\begin{alignat}{6}
\opt^p \geq \min &&~\sum_{v,u \in X} d(v,u)^p x_{vu}  \tag{LP}\label{lp:ppkc}\\
&& \sum_{u \in X}x_{vu} ~=~ 1, && ~~\forall v \in X &\tag{LP1}\label{lp:cover} \\
&& \sum_{u \in X} y_u ~=~ k & \tag{LP2}\label{lp:budget}
\end{alignat}
\end{minipage}
\begin{minipage}{0.45\textwidth}
\begin{alignat}{6}
&& x_{vu} ~\leq~ y_u, && ~\forall v,u \in X\tag{LP3}\label{lp:open}\\ 
&& x_{vu} ~=~  0, && ~\forall v,u : d(v,u) > r(v) \tag{LP4}\label{lp:connect}\\
&& 0 \leq x_{vu}, y_u  ~\leq~ 1, &&~~ \forall v,u \in X.\notag
\end{alignat}
\end{minipage}

% \begin{align}
% \min \sum_{v,u \in X} d(v,u)^p&x_{vu} & \tag{ LP}\label{lp:ppkc}\\
% \sum_{u \in X}x_{vu} =& 1 & \forall v \in X\tag{LP1}\label{lp:cover}\\
% \sum_{u \in X} y_u =& k & \tag{LP2}\label{lp:budget}\\
% x_{vu} \leq& y_u & \forall v,u \in X\tag{LP3}\label{lp:open}\\ 
% x_{vu} =&  0 & \forall v,u \in X: d(v,u) > r(v) \tag{LP4}\label{lp:connect}\\
% 0 \leq x_{vu}, y_u  \leq& 1 & \forall v,u \in X.\notag
% \end{align}

From here on, we use the notation $B(u,r)$ for $u \in X$ and $r \in \Rset^+$ to denote the points in a ball of radius $r$ around $u$. That is $B(u,r) := \{v \in X: d(u,v) \leq r\}$. Also, for any set of points $U \subseteq X$, let $y(U):= \sum_{u\in U}y_u$. Considering \eqref{lp:connect} and \eqref{lp:cover} the following holds.
\begin{fact}\label{fact:lpyis1}
If $y$ is from a feasible \ref{lp:ppkc} solution, then $y(B(v,r(v))) \geq 1$ for all $v\in X$.
\end{fact}

We now describe a routine \filter due to \cite{Ples87,hs85} which is used as a subroutine in our main algorithm. Assume all the points are initially ``uncovered''. The routine takes a function $R: X \to \Rset^+$, sorts the points in order of {\em increasing} $R(v)$'s. Then it considers the first point in this order, calls it a ``representative'' and ``covers'' all the points $v$ at distance at most $2r(v)$ from it. Call these points $D(v)$.
Repeating this procedure until all the points are covered, forms a partition on $X$ such that the representatives are ``far apart'', while each non-representative is assigned to a ``nearby'' representative, among other useful properties listed in \Cref{fact:filter} and \Cref{fact:coreinside}.
\begin{algorithm}[ht]
	\caption{\filter}
	\label{alg:filter}
	\begin{algorithmic}[1]
		\Require Metric $(X,d)$, radius function $R: X \to \Rset^+$
		\State $U \leftarrow X$ \Comment{The set of ``uncovered points''} \label{ln:1}
		\State $S \leftarrow \emptyset$ \Comment{The set of ``representatives''}
		\While{ $U \neq \emptyset$}
	        \State $u \leftarrow \arg\min_{v\in U} R(v)$ \Comment{The first point in $U$ in non-decreasing $R$ order}  \label{ln:greedy}
	        \State $S \leftarrow S \cup u$ \label{ln:rep}
	        \State $D(u) \leftarrow \{v \in U: d(u,v) \leq 2R(v)\}$\Comment{$D(u) = B(u,2R(v))\cap U$ and includes $u$ itself} \label{ln:chld}
	        \State $U \leftarrow U \backslash D(u)$ \label{ln:remove-from-U}
		\EndWhile
		\Ensure $S$, $\{D(u) : u \in S\}$
	\end{algorithmic}
\end{algorithm}

\begin{fact}\label{fact:filter}\cite{Ples87,hs85} 
The following is true for the output of \filter: (a) $\forall u,v \in S, d(u,v) > 2\max\{R(u),R(v)\}$, (b) The balls $\{B(u,R(u)) : u \in S\}$ are mutually disjoint, (c) The set $\{D(u) : u \in S\}$ partitions $X$, (d) $\forall{u \in S},\forall{v \in D(u)}, R(u) \leq R(v)$, and (e) $\forall{u \in S},\forall{v \in D(u)}, d(u,v) \leq 2R(v)$.
% \begin{itemize}
%     \item $\forall u,v \in S, d(u,v) > 2\max\{R(u),R(v)\}$.
%     \item The balls $\{B(u,R(u)) : u \in S\}$ are mutually disjoint.
%     \item The set $\{D(u) : u \in S\}$ partitions $X$.
%     \item $\forall{u \in S},\forall{v \in D(u)}, R(u) \leq R(v)$.
%     \item $\forall{u \in S},\forall{v \in D(u)}, d(u,v) \leq 2R(v)$.
% \end{itemize}
\end{fact}

\begin{fact}\label{fact:coreinside}
For any $u \in S$ and $w \in B(u,R(u))$, the unique closest point in $S$ to $w$ is $u$.
\end{fact}
\begin{proof}
Suppose otherwise. That is, there exists $v \in S$ not equal to $u$ s.t. $d(w,v) \leq d(w,u)$. Then $d(u,v) \leq d(u,w) + d(w,v) \leq 2d(w,u) \leq 2R(u)$ which contradicts \Cref{fact:filter} as we must have $d(u,v) > 2\max\{R(u),R(v)\}$.
\end{proof}

To elaborate on the importance of \Cref{alg:filter} and build some intuition, we point out the following theorem of ~\cite{Ples87,JKL20}.
\begin{theorem}\label{thm:ples}
Take $S$ the output of \Cref{alg:filter} on a \ppkc instance with $R := r$. Then if the instance is feasible, $|S| \leq k$ and $d(v,S) \leq 2r(v)$ for all $v \in X$.
\end{theorem}
\begin{proof}
By \Cref{fact:filter} we know that $\{D(u) : u \in S\}$ partitions $X$ so for any $v \in X$, there exists a $u\in S$ for which $v \in D(u)$. Plus, $d(v,u) \leq 2R(v) = 2r(v)$. Now it only remains to prove $|S| \leq k$. To see this, let $S^*$ be some feasible solution and observe that two different $u,w \in S$, cannot be covered by \emph{the same} center in $S^*$. Since otherwise, if there exists $f \in S^*$ for which $d(u,f) \leq r(u)$ and $d(w,f) \leq r(w)$ by triangle inequality $d(u,v) \leq d(u,f) + d(f,w) \leq r(u) + r(v)$ and this contradicts $d(u,w) > 2\max\{r(u),r(v)\}$ from \Cref{fact:filter}.
\end{proof}

But of course, the above theorem does not give any guarantees for the clustering cost (unless $p = \infty$). It might be the case that many points are paying close to 0 towards the clustering cost in the optimal solution, but are made to connect to a point much farther in the above procedure. 

==> Priority k-Median(3)/starter.tex <==
\usepackage{amsthm,amssymb,amsmath}
\usepackage{algorithm}
\usepackage{algpseudocode}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\usepackage{graphicx}

\usepackage[nameinlink]{cleveref}

\newtheorem{theorem}{Theorem}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{fact}{Fact}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem	{itheorem}{Result}
\crefname{Fact}{Fact}{Facts}

\usepackage{xspace}


\newcommand{\Rset}{\mathbb{R}}


\newcommand{\norm}[1]{\left\lVert#1\right\rVert}


\newcommand{\modas}{\textsf{mod-AS}\xspace}
\newcommand{\relaxedmodas}{\textsf{relaxed-mod-AS}\xspace}
\newcommand{\sparsemodas}{\textsf{sparse-mod-AS}\xspace}
\newcommand{\opt}{\textsf{opt}\xspace}
\newcommand{\lpnorm}{{$\ell_p$-norm}\xspace}
\newcommand{\cost}{{$\big(\sum_{v \in X} d(v,S)^p\big)^{1/p}$}}
\newcommand{\ourbeta}{{2^{1+2/p}}}

\newcommand{\kcentmed}{\textsc{$k$-(Center,Median)}\xspace}
\newcommand{\kcent}{\textsc{$k$-Center}\xspace}
\newcommand{\kmeans}{\textsc{$k$-Means}\xspace}
\newcommand{\kmed}{\textsc{$k$-Median}\xspace}
\newcommand{\pkmeans}{\textsc{Fair-$k$-Means}\xspace}
\newcommand{\pkmed}{\textsc{Fair-$k$-Median}\xspace}
\newcommand{\pkcent}{\textsc{Fair-$k$-Center}\xspace}
\newcommand{\ppkc}{\textsc{Fair-$(p,k)$-Clustering}\xspace}
\newcommand{\pkc}{\textsc{$(p,k)$-Clustering}\xspace}

\newcommand{\filter}{\textsf{Filter}\xspace}
\newcommand{\algoname}{\textsf{Fair-Round}\xspace}
\newcommand{\relalgoname}{\textsf{Relaxed-Fair-Round}\xspace}
\newcommand{\spaalgoname}{\textsf{Sparse-Fair-Round}\xspace}
\newcommand{\kmeanspp}{\textsf{$k$-Means$++$}\xspace}
\newcommand{\lskmeans}{\textsf{LS-$k$-Means}\xspace}

\def\bank{{\tt bank}\xspace}
\def\census{{\tt census}\xspace}
\def\diabetes{{\tt diabetes}\xspace}
\def\creditcard{{\tt creditcard}\xspace}
\def\censusbig{{\tt census1990}\xspace}

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{We have provable guarantees}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{In references for the ones named in paper, in comments of the codes for the rest.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Snippets of code. credited in code comments}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> conclusion.tex <==
\section{Conclusion}

